\epsilon-regularity for systems involving non-local, antisymmetric operators

We prove an epsilon-regularity theorem for critical and super-critical systems with a non-local antisymmetric operator on the right-hand side. These systems contain as special cases, Euler-Lagrange equations of conformally invariant variational functionals as Rivi\`ere treated them, and also Euler-Lagrange equations of fractional harmonic maps introduced by Da Lio-Rivi\`ere. In particular, the arguments presented here give new and uniform proofs of the regularity results by Rivi\`ere, Rivi\`ere-Struwe, Da-Lio-Rivi\`ere, and also the integrability results by Sharp-Topping and Sharp, not discriminating between the classical local, and the non-local situations.

==> regp.tex <==
\section{Morrey-Regularity for the Frame}
We hope to show that the minimizer $P$ from Lemma \ref{la:energy:Pmineuler}, which is a priori supposed to satisfy $P \in L^\infty(\R^m)$, $\laps{\mu} P \in L^2(\R^m)$ actually satisfies
\[
 \sup_{B_\rho \subsubset D} \rho^{\sigma-m}\vrac{\laps{\mu} P}_{2,B_\rho} < \infty,
\]
for $\sigma > \mu$ as close as possible to $\mu$.\\
Assume that $\Omega[] = A\Rz[]$, and
\[
\begin{ma}
- \int \Omega^P[\laps{\mu} \varphi]
 &=& \fracm{2} \int H_{\mu}(P-I,P^T-I)\ \laps{\mu} \varphi\\
 &&-\int so(P\mathcal{C}\brac{\varphi, \Omega}\left [P^T \overline{\Omega^P}^T \chi_{D_\Lambda}\right ])  \\
&& + \int so(\overline{\Omega^P} \chi_{D_\Lambda}P H_{\mu}(\varphi,P^T-I))\\
&& - \int so(\mathcal{C}\brac{P,\Omega}[\laps{\mu} \varphi] P^T).
\end{ma}
\]
Since
\[
\Omega^Q [\laps{\mu} \varphi]:= \brac{\laps{\mu} (Q-I)}\ Q^T\ \laps{\mu} \varphi + Q \Omega [Q^T \laps{\mu} \varphi],
\]
we have for all $\varphi \in C_0^\infty(D)$,
\[
\begin{ma}
- \int \brac{\laps{\mu} Q}\ Q^T\ \laps{\mu} \varphi  &=& \int Q \Omega [Q^T \laps{\mu} \varphi] \\
 &&+\fracm{2} \int H_{\mu}(P-I,P^T-I)\ \laps{\mu} \varphi\\
 &&-\int so(P\mathcal{C}\brac{\varphi, \Omega}\left [P^T \overline{\Omega^P}^T \chi_{D_\Lambda}\right ])  \\
&& + \int so(\overline{\Omega^P} \chi_{D_\Lambda}P H_{\mu}(\varphi,P^T-I))\\
&& - \int so(\mathcal{C}\brac{P,\Omega}[\laps{\mu} \varphi] P^T).
\end{ma}
\]
Assume that
\eqref{eq:regp2} holds
\begin{equation}
 \label{eq:regp2}
 \sup_{B_\rho(x), x \in D} \sup_{\psi \in C_0^\infty{B_\rho(x)}}\ \vrac{\psi}_2^{-1}\ \rho^{2\mu-m}\vrac{\Omega[\psi]}_{L^1} \leq \theta
\end{equation}
 

\begin{theorem}
Under these conditions, also for any $\tilde{D} \subsubset D$, $\sigma \in (2\mu,m]$, \ToDo if $2\mu = m$
\begin{equation}
 \sup_{B_\rho(x), x \in D} \sup_{\psi \in C_0^\infty{B_\rho(x)}}\ \vrac{\psi}_2^{-1}\ \rho^{\sigma-m}\vrac{\Omega[\psi]}_{L^1} \leq C_{\tilde{D},\sigma}\ \Theta
\end{equation}
\end{theorem}
